Compact Routing Messages in Self-Healing Trees

Existing compact routing schemes, e.g., Thorup and Zwick [SPAA 2001] and Chechik [PODC 2013], often have no means to tolerate failures, once the system has been setup and started. This paper presents, to our knowledge, the first self-healing compact routing scheme. Besides, our schemes are developed for low memory nodes, i.e., nodes need only $O(\log^2 n)$ memory, and are thus, compact schemes. We introduce two algorithms of independent interest: The first is CompactFT, a novel compact version (using only $O(\log n)$ local memory) of the self-healing algorithm Forgiving Tree of Hayes et al. [PODC 2008]. The second algorithm (CompactFTZ) combines CompactFT with Thorup-Zwick's tree-based compact routing scheme [SPAA 2001] to produce a fully compact self-healing routing scheme. In the self-healing model, the adversary deletes nodes one at a time with the affected nodes self-healing locally by adding few edges. CompactFT recovers from each attack in only $O(1)$ time and $\Delta$ messages, with only +3 degree increase and $O(log \Delta)$ graph diameter increase, over any sequence of deletions ($\Delta$ is the initial maximum degree). Additionally, CompactFTZ guarantees delivery of a packet sent from sender s as long as the receiver t has not been deleted, with only an additional $O(y \log \Delta)$ latency, where $y$ is the number of nodes that have been deleted on the path between $s$ and $t$. If $t$ has been deleted, $s$ gets informed and the packet removed from the network.

==> Abstract.tex <==
% !TEX root = SHRoutingDISC15.tex

\begin{abstract}

Existing compact routing schemes (For example, by Thorup and Zwick [SPAA 2001] and by Chechik [PODC 2013]) often have no mechanism for tolerating failures, once the routing system has been setup and started. This paper presents, to our knowledge, the first self-healing compact routing scheme. Our schemes are  developed for low memory nodes \ie nodes need only use $O(\log n)$ memory, and are thus, compact schemes. 

We introduce two algorithms of independent interest: The first is \emphCFT, a novel compact version of the self-healing algorithm \emph{Forgiving Tree} of Hayes et al. [PODC 2008]. The second algorithm (\emphtzft) combines CompactFT with Thorup-Zwick's tree-based compact routing scheme [SPAA 2001] to produce a fully compact self-healing routing scheme.  Our algorithms work in the self-healing model where a powerful adversary deletes nodes from the network one at a time and on each deletion, the neighbours of the deleted node self-heal the network locally by adding a small number of edges. CompactFT ensures recovery from each attack in only a constant time and $\Delta$ messages, while,  over any sequence of deletions, taking only constant additive degree increase (of 3) and $O(\log \Delta)$ graph diameter increase, where $\Delta$ is the maximum degree in the initial spanning tree.
$\tzft$  guarantees delivery of a packet sent from sender $s$ as long as the receiver $t$ has not been deleted, with only an additional  $O(y \log \Delta)$ latency, where  $y$ is the number of nodes that have been deleted on the path between $s$ and $t$.

%Our routing algorithm ensures routing between any pair of existing nodes in our self-healing tree without loss of any message packets. Moreover, the source will be informed if the receiver is no more and if both the sender and receiver have been lost,  the message will be discarded from the system within at most twice of the routing time. Our algorithm guarantees that after $x$ deletions, a packet from $s$ to $t$ is routed through a path of length at most $d(s,t) + O(x \log \Delta)$, where $d(s,t)$ is the distance between $s$ and $t$ in the initial tree. 


%Our algorithm guarantees that even under adversarial attack, the algorithm self-heals and routing between any pair of existing nodes remains available and none of the packets are lost by the algorithm. Any packet originating at node $s$ for node $t$ will be delivered at node $t$ if node $t$ exists; if node $t$ has been deleted, node $s$ will be informed by the algorithm of the non-delivery, and if node $s$ has also been deleted in the meanwhile, the message will be discarded from the system within at most twice of the routing time. Our algorithm guarantees that after $x$ deletions, a packet from $s$ to $t$ is routed through a path of length at most $d(s,t) + O(x \log \Delta)$, where $d(s,t)$ is the distance between $s$ and $t$ in the initial tree and $\Delta$ is the maximum degree in the initial tree. Further, recovery from each attack takes only constant time and constant number of messages and over all deletions, nodes may increase their degree by at most 3.

%We present a scheme that uses local memory proportional to $\Delta$ and thus may not be compact for all topologies. However, for our final universally compact scheme, we devise a compact  Forgiving Tree implementation (using only $polylog(n)$ local memory), which is of independent interest itself.

\iffalse
%A \emph{routing scheme} is a distributed algorithm that allows the nodes of a network $G$, modeled as a graph, to route a packet $M$ from any node $u$ to any node $v$. Each node in the path $M$ traverses decides the next node using local information, called its \emph{routing table}, and some information added to $M$, its \emph{header}. In a \emph{compact} routing scheme, routing tables and headers are sub-linear in the number of nodes~$n$.

%%We are interested in compact routing schemes with a \emph{good that route a packets
%%between $u$ and $v$ through a path that is not much larger than the distance between 
%%$u$ and $b$ in $G$, for any nodes $u,v$.

%Several routing schemes have been proposed (For example, by Thorup and Zwick [SPAA 2001] and by Chechik [PODC 2013]). However none of them is fault tolerant.
%All of them follow a rigid structure in which they compute local tables and headers in a pre-processing stage and then in a second stage the actual distributed algorithm  starts routing messages. But there is no mechanism for tolerating failures once the system has started.

Existing compact routing schemes (For example, by Thorup and Zwick [SPAA 2001] and by Chechik [PODC 2013]) are not fault-tolerant. They follow a rigid structure in which they compute local tables and headers in a pre-processing stage and then in a second stage the actual distributed algorithm  starts routing messages. But there is no mechanism for tolerating failures once the system has started. This paper presents the first fault-tolerant compact routing schemes. Our algorithms are based on tree-based compact routing schemes of Thorup and Zwick [SPAA 2001] and on a novel compact version of the self-healing algorithm \emph{Forgiving Tree} of Hayes et al. [PODC 2008]. 


%The Forgiving Tree (FT) is a self-healing distributed data structure initialized on a spanning tree of the network; a powerful adversary deletes nodes one at a time and on each deletion, the remaining nodes self-heal the network by adding a small number of edges. FT maintains connectivity and distances with only additive constant degree increase over the whole series of deletion while taking only constant time and messages per deletion. In our algorithm, after a deletion of a node there is a recovery phase inwhich the connectivity of the tree is restored, and then routing among any  pair of remaining nodes is still available.

Our algorithm is in the self-healing model where a powerful adversary deletes nodes from the network one at a time and on each deletion, the remaining nodes self-heal the network by adding a small number of edges.
Our algorithm guarantees that even under adversarial attack, the algorithm self-heals and routing between any pair of existing nodes remains available and none of the packets are lost by the algorithm. Any packet originating at node $s$ for node $t$ will be delivered at node $t$ if node $t$ exists; if node $t$ has been deleted, node $s$ will be informed by the algorithm of the non-delivery, and if node $s$ has also been deleted in the meanwhile, the message will be discarded from the system within at most twice of the routing time. Our algorithm guarantees that after $x$ deletions, a packet from $s$ to $t$ is routed through a path of length at most $d(s,t) + O(x \log \Delta)$, where $d(s,t)$ is the distance between $s$ and $t$ in the initial tree and $\Delta$ is the maximum degree in the initial tree. Further, recovery from each attack takes only constant time and constant number of messages and over all deletions, nodes may increase their degree by at most 3.

We present a scheme that uses local memory proportional to $\Delta$ and thus may not be compact for all topologies. However, for our final universally compact scheme, we devise a compact  Forgiving Tree implementation (using only $polylog(n)$ local memory), which is of independent interest itself.

\fi

\end{abstract}

